The ALICE TPC, a large 3-dimensional tracking device with fast readout for ultra-high multiplicity events

The design, construction, and commissioning of the ALICE Time-Projection Chamber (TPC) is described. It is the main device for pattern recognition, tracking, and identification of charged particles in the ALICE experiment at the CERN LHC. The TPC is cylindrical in shape with a volume close to 90 m^3 and is operated in a 0.5 T solenoidal magnetic field parallel to its axis. In this paper we describe in detail the design considerations for this detector for operation in the extreme multiplicity environment of central Pb--Pb collisions at LHC energy. The implementation of the resulting requirements into hardware (field cage, read-out chambers, electronics), infrastructure (gas and cooling system, laser-calibration system), and software led to many technical innovations which are described along with a presentation of all the major components of the detector, as currently realized. We also report on the performance achieved after completion of the first round of stand-alone calibration runs and demonstrate results close to those specified in the TPC Technical Design Report.

==> tpcnimpackages.tex <==
\biboptions{sort&compress,square,comma}

\ifpdf
  \PassOptionsToPackage{pdftex}{graphicx}
\else
  \PassOptionsToPackage{dvips}{graphicx}
\fi
\RequirePackage{graphicx}
%
\usepackage{booktabs}
\usepackage{xspace}
\usepackage{float}
\floatplacement{figure}{H} %
\floatplacement{table}{H} %
%
\usepackage[format=hang,font=small,labelfont=bf,margin=10pt]{subfig} %
\captionsetup[subfigure]{font=footnotesize}
\usepackage{latexsym}
\usepackage{amsmath,amssymb,textcomp,amsfonts}
%
%
%
\usepackage{calc}
\usepackage{acronym}
\usepackage{color}
\usepackage[english]{babel}
\usepackage{multirow}
\usepackage{longtable}

\usepackage[amssymb]{SIunits}
\addunit{\bit}{bit} %
\addunit{\byte}{Byte} %
\addunit{\lsb}{LSB}
\addunit{\msps}{MSPS}


\definecolor{darkblue}{rgb}{0,0,.3}

\ifpdf
  \usepackage[pdftex,colorlinks=true]{hyperref}
  \pdfcompresslevel=9     %
\else
  \usepackage[ps2pdf,colorlinks=false, pdfborder={0 0 0}]{hyperref}
\fi

\hypersetup{ 
  pdfauthor={ALICE Collaboration}, 
  pdftitle={The ALICE Time Projection Chamber}, 
  pdfsubject={Paper},
  pdfproducer={LaTeX},
  citecolor=green,
  linkcolor=darkblue,   %
%
  urlcolor=blue,   %
  breaklinks=true,   %
%
  pdfhighlight=/I
%
}


%
\newcommand{\thead}[1]{\multicolumn{1}{c}{\bf #1}}
\newcommand{\HRule}{\rule{0.4\linewidth}{0.3mm}}


